Chronodes: Interactive Multi-focus Exploration of Event Sequences

The advent of mobile health technologies presents new challenges that existing visualizations, interactive tools, and algorithms are not yet designed to support. In dealing with uncertainty in sensor data and high-dimensional physiological records, we must seek to improve current tools that make sense of health data from traditional perspectives in event-based trend discovery. With Chronodes, a system developed to help researchers collect, interpret, and model mobile health (mHealth) data, we posit a series of interaction techniques that enable new approaches to understanding and exploring event-based data. From numerous and discontinuous mobile health data streams, Chronodes finds and visualizes frequent event sequences that reveal common chronological patterns across participants and days. By then promoting the sequences as interactive elements, Chronodes presents opportunities for finding, defining, and comparing cohorts of participants that exhibit particular behaviors. We applied Chronodes to a real 40GB mHealth dataset capturing about 400 hours of data. Through our pilot study with 20 behavioral and biomedical health experts, we gained insights into Chronodes' efficacy, limitations, and potential applicability to a wide range of healthcare scenarios.

==> 850implications.tex <==
\tod{frequence, progressive vis}

\tod{this section is highly redundant. most everything described in it is already addressed explicitly in the results section.}

In this section, we use insights learned from our experience with Chronodes to provide recommendations for future work on mHealth data visualization and inference.
% describe potential directions of work in healthcare interface development, as well as open questions and challenges, that we have identified during our work with Chronodes.
% These findings summarize recommendations for future work in representing mHealth data develop.
% \tod{guide, offer recommendations, inspire, precursor to future contributions to mHealth data visualization and inference / design}

% \moushumi{some points is a summary of ``imporvements'' above; some points are general, high-level challenges that are open problems}
% \moushumi{list challenges and say we address a few here. There are a lot of open problems.}

\subsubsection{Defining Events}

% All things considered, the benefits of representing time-series data as discrete events may be insufficient for mHealth data, where computational data mining and modeling is becoming increasingly relevant.
As machine learning algorithms like frequent sequence mining in Chronodes are more readily applied to mHealth data analysis, we are presented with new opportunities for observing health data from non-discrete, non-linear perspectives.
% \tod{new opportunities for quantifying / determining behavior from data mining and machine learning perspectives}
% \tod{most existing algorithms can only handle discrete events in the first place}
% \tod{like ours and others'}
Chronodes uses Boolean values and thresholds on quantitative values to define discrete events, and employs sequence mining on these events to reveal their interrelationships.
Still, this is only one approach to modeling mHealth data, and many more opportunities exist for
describing time-series mHealth data from other perspectives in machine learning.
Interpreting health data in terms of, for example, temporal features \cite{Gschwandtner:2011:carecruiser} or probabilistic motifs \cite{Chiu:2003:probabilistic} are alternate routes of analysis that take advantage non-discrete mHealth data properties.
% Particularly in seeking to represent uncertain events and latent variables, defining events as discrete entities 

% Participant D also proposed the critically useful suggestion of ranking frequent sequences by conditional frequency.
% As opposed to simply ranking sequences by their frequency within the observed cohort, it is additionally useful to see how this frequency compares to that of participants \textit{outside} of the cohort at hand.

\subsubsection{Scaling to More Dimensions}

Representing multiple events simultaneously suggests a challenge for scaling to more sensor kinds.
Although Chronodes is designed to handle the integration of multiple sensors, like other existing timeline tools in healthcare it cannot yet depict many sensor data streams, for many participants, at once.
This problem of dimensional scalability is perhaps the greatest and most interesting in designing visualizations for this field.
% For hundreds or thousands of participants, certainly all health data streams do not need to be visualized explicitly---
% which should be left out, or how should they be integrated together?
% The inclusion of multiple participants The fundamental interactive techniques and algorithms designed into Chronodes are applicable to any number of participants, but the system's visual representation of participant data will need to be modified as we scale to larger datasets.
% Particularly in the \Orchestra, instead of visualizing each participants' event data explicitly we must seek to cluster participants into groups or represent them with more compact visual summaries \cite{eamonn2005time}.


\subsubsection{Clarifying Frequent Sequence Mining}

To Participant G, the concept of frequent sequence mining was intuitive once introduced, but the notion of allowing `gaps' between \textit{focal} sequences was unfamiliar.
Although our team has discussed options for defining parameters like maximum gaps in great detail, more work needs to be done to balance algorithm effectiveness with comprehensibility.
